Towards a Formalisation of Justification and Justifiability

We introduce the logic QKSD which is a normal multi-modal logic over finitely many modalities that additionally supports bounded quantification of modalities. An important feature of this logic is that it allows to quantify over the information components of systems and, hence, can be used to derive justifications. We compare the proposed logic with Artemov's justification logic and also report on a prototypical implementation of a satisfiability solver of this logic and show some examples.

==> eptcsdata.tex <==
\providecommand{\firstpage}{136}
\providecommand{\publicationstatus}{M. Farrell \& M. Luckcuck (Eds.): \\Third Workshop
on Formal Methods \\for Autonomous Systems (FMAS2021)\\
EPTCS 348, 2021, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.348.10}{10.4204/EPTCS.348.10}}
\pdfoutput=1

